Cubical Approximation for Directed Topology II

The paper establishes an equivalence between directed homotopy categories of (diagrams of) cubical sets and (diagrams of) directed topological spaces. This equivalence both lifts and extends an equivalence between classical homotopy categories of cubical sets and topological spaces. Some simple applications include combinatorial descriptions and subsequent calculations of directed homotopy monoids and directed singular 1-cohomology monoids. Another application is a characterization of isomorphisms between small categories up to zig-zags of natural transformations as directed homotopy equivalences between directed classifying spaces. Cubical sets throughout the paper are taken to mean presheaves over the minimal symmetric monoidal variant of the cube category. Along the way, the paper characterizes morphisms in this variant as the interval-preserving lattice homomorphisms between finite Boolean lattices.

==> notation.tex <==
% novel to approx_II paper:

\newcommand{\BOX}{\square}
\newcommand{\ORIENTEDBOX}{\BOX_{\circlearrowright}}

\mathchardef\mhyphen="2D

\DeclareMathAlphabet{\callrsfs}{OT1}{pzc}{m}{it} 

\makeatletter
\newcommand{\dashover}[2][\mathop]{#1{\mathpalette\df@over{{\dashfill}{#2}}}}
\newcommand{\df@over}[2]{\df@@over#1#2}
\newcommand\df@@over[3]{%
  \vbox{
    \offinterlineskip
    \ialign{##\cr
      #2{#1}\cr
      \noalign{\kern1pt}
      $\m@th#1#3$\cr
    }
  }%
}
\newcommand{\dashfill}[1]{%
  \kern-.5pt
  \xleaders\hbox{\kern.5pt\vrule height.4pt width \dash@width{#1}\kern.5pt}\hfill
  \kern-.5pt
}
\newcommand{\dash@width}[1]{%
  \ifx#1\displaystyle
    2pt
  \else
    \ifx#1\textstyle
      1.5pt
    \else
      \ifx#1\scriptstyle
        1.25pt
      \else
        \ifx#1\scriptscriptstyle
          1pt
        \fi
      \fi
    \fi
  \fi
}
\makeatother

% general
\newcommand{\I}{\mathbb{I}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\K}{\mathbb{K}}

% formatting
\newcommand{\backspace}{\!\!\!\!\!\!\!}
\newcommand{\upsidedown}[1]{\reflectbox{\rotatebox[origin=c]{180}{#1}}}
\newcommand\circumscribe[1]{\stackMath\mathbin{\stackinset{c}{0ex}{c}{0ex}{#1}{\bigcirc}}}
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}

% greek
\newcommand{\Tau}{\mathrm{T}}
\newcommand{\Iota}{\mathrm{I}}

% category theory
\newcommand{\codomain}{\catfont{cod}}
\newcommand{\domain}{\catfont{dom}}
\newcommand{\catfont}[1]{\mathrm{\bf #1}}
\newcommand{\coequalizer}[5]{\xymatrix@C=6pc{#1\ar@<.7ex>[r]^{#4}\ar@<-.7ex>[r]_{#5} & #2\ar@{.>}[r] & #3}}
\newcommand{\forget}{\catfont{forget}}
\newcommand{\smallcat}[1]{\ifthenelse{1=#1}{\mathcal{X}}{\ifthenelse{2=#1}{\mathcal{Y}}{\mathcal{Z}}}}
\newcommand{\smallgroupoid}[1]{\ifthenelse{1=#1}{\mathcal{G}}{\mathcal{H}}}
\newcommand{\modelcat}[1]{\ifthenelse{1=#1}{\mathscr{M}}{\ifthenelse{2=#1}{\mathscr{N}}{\mathscr{O}}}}
\newcommand{\reedycat}[1]{\ifthenelse{1=#1}{\mathscr{R}}{\ifthenelse{2=#1}{\mathscr{S}}{\mathscr{T}}}}
\newcommand{\cat}[1]{\ifthenelse{1=#1}{\mathscr{X}}{\ifthenelse{2=#1}{\mathscr{Y}}{\mathscr{Z}}}}
\newcommand{\shape}[1]{\ifthenelse{1=#1}{{\small\bigcirc}}{\ifthenelse{2=#1}{{\large\pentagon}}{\octagon}}}
\newcommand{\doublecat}[1]{\ifthenelse{1=#1}{\mathscr{C}}{\ifthenelse{2=#1}{\mathscr{D}}{\mathscr{E}}}}
\newcommand{\doublefunctor}[1]{\ifthenelse{1=#1}{\mathfrak{F}}{\ifthenelse{2=#1}{\mathfrak{G}}{\mathfrak{H}}}}
\newcommand{\BASED}[1]{#1_{\star}}
\newcommand{\adjoint}{\catfont{adj}}
\newcommand{\Aut}{\mathop{Aut}}
\newcommand{\Hom}{\mathop{Hom}}
\newcommand{\la}{\leftarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\rras}{\rightrightarrows}
\newcommand{\partialra}{\rightharpoonup}
\newcommand{\xra}{\xrightarrow}
\newcommand{\xla}{\xleftarrow}
\newcommand{\xira}{\xhookrightarrow}
\newcommand{\lras}{\leftrightarrows}
\newcommand{\ira}{\hookrightarrow}
\newcommand{\epi}{\twoheadrightarrow}
\newcommand{\colim}{\mathrm{colim}}
\newcommand{\holim}{\mathrm{holim}}
\newcommand{\hocolim}{\mathrm{hocolim}}
\newcommand{\id}{1}
\newcommand{\im}{{\catfont{im}}}
\newcommand{\counit}{\epsilon}
\newcommand{\unit}{\eta}
\newcommand{\pullback}[1]{{#1}^*}
\newcommand{\pushforward}[1]{{#1}_*}
\newcommand{\cardinality}{\#}
\newcommand{\OP}[1]{#1^{\mathrm{op}}}
\newcommand{\WE}{\mathop{h}}
\newcommand{\DERIVED}{\mathscr{D}}
\newcommand{\PAIRS}[1]{(#1,#1)}
\newcommand{\CUBICAL}{\catfont{c}}
\newcommand{\REEDY}{\mathscr{R}}
\newcommand{\SIMPLICIAL}{\catfont{s}}
\newcommand{\BI}[1]{#1 #1}
\newcommand{\GENERIC}{\mathscr{X}}
\newcommand{\SMALLGENERIC}{\mathcal{X}}
\newcommand{\PREORDEREDSETS}{\mathscr{Q}}
\newcommand{\SEMIMODULES}{\mathscr{M}}
\newcommand{\ALGEBRAS}[1]{\catfont{Alg}_{#1}}
\newcommand{\CATS}{\catfont{Cat}}%{\calligra{Cat}}
\newcommand{\DOUBLECATS}{\calligra{Cat^{(2)}}}%{\calligra{Cat}}
\newcommand{\GROUPOIDS}{\catfont{Gpd}}%{\calligra{Cat}}
\newcommand{\OMEGAGROUPOIDS}{\omega\GROUPOIDS}%{\calligra{Cat}}
\newcommand{\OMEGACATS}{\omega\CATS}%{\calligra{Cat}}
\newcommand{\indexcat}[1]{{\ifthenelse{1=#1}{\mathscr{G}}{{\ifthenelse{2=#1}{\mathscr{H}}{\mathscr{I}}}}}}
\newcommand{\DEL}{\Delta}
\newcommand{\MONOIDAL}{\mathscr{V}}
\newcommand{\SEMIAB}{\mathscr{A}}
\newcommand{\Sh}{\mathop{Sh}\;\!\!\!}
\newcommand{\sheafification}{\callrsfs{Sheaf}}
\newcommand{\kernel}{\mathrm{ker}}
\newcommand{\cokernel}{\mathrm{cok}}
\newcommand{\nullity}{\mathrm{null}}
\newcommand{\quotient}[2]{{\raisebox{.2em}{$#1$}\left/\raisebox{-.2em}{$#2$}\right.}}
\newcommand{\PRESHEAVES}[1]{\hat{#1}}
\newcommand{\MULTIPOINTED}[1]{{#1}_{\star\cdots\star}}
\newcommand{\VECTORSPACES}{\catfont{Vec}}
\newcommand{\AFFINESPACES}{\catfont{Aff}}
\newcommand{\POSETS}{\catfont{Pos}}
\newcommand{\QUASIUNIFORM}{\mathscr{Q}}
\newcommand{\UNIFORM}{\mathscr{U}}
\newcommand{\HEMIMETRICSPACES}{\catfont{Hem}}
\newcommand{\BANACH}{\mathscr{B}}
\newcommand{\MODULES}{\mathscr{M}}
\newcommand{\COALGEBRAS}{\mathrm{Coalg}}
\newcommand{\HOMOTOPY}{h}
\newcommand{\Ch}{\mathop{Ch}\;\!\!}
\newcommand{\SEMICHAINS}{\mathop{ch}\;\!\!}

\newcommand{\TOP}{\catfont{Top}}
\newcommand{\STREAMS}{\catfont{Str}}
\newcommand{\DITOP}{\catfont{DiTop}}
\newcommand{\FINITESETS}{\catfont{FinSet}}
\newcommand{\SETS}{\catfont{Set}}
\newcommand{\BOOLEAN}{\catfont{Bool}}
\newcommand{\RELATIONS}{\catfont{Rel}}
\newcommand{\PROOBJECTS}[1]{\catfont{pro}\mhyphen #1}

% arithmetic
\newcommand{\half}{\nicefrac{1}{2}}
\newcommand{\third}{\nicefrac{1}{3}}
\newcommand{\fourth}{\nicefrac{1}{4}}
\newcommand{\fifth}{\nicefrac{1}{5}}
\newcommand{\sixth}{\nicefrac{1}{6}}
\newcommand{\seventh}{\nicefrac{1}{7}}
\newcommand{\eight}{\nicefrac{1}{8}}
\newcommand{\ninth}{\nicefrac{1}{9}}

% algebra
\newcommand{\threebythree}[9]{\left(\begin{tabular}{ccc}#1&#2&#3\\#4&#5&#6\\#7&#8&#9\end{tabular}\right)}  
\newcommand{\twobythree}[6]{\left(\begin{tabular}{ccc}#1&#2&#3\\#4&#5&#6\end{tabular}\right)}  
\newcommand{\threebytwo}[6]{\left(\begin{tabular}{cc}#1&#2\\#3&#4\\#5&#6\end{tabular}\right)}  
\newcommand{\twobytwo}[4]{\left(\begin{tabular}{cc}#1&#2\\#3&#4\end{tabular}\right)}  
\newcommand{\semidirectproduct}{\rtimes}
\newcommand{\conjugate}[2]{\;\!^{#2}\!#1}
\newcommand{\ZPLUS}{\Z^+}
\newcommand{\ring}[1]{{\ifthenelse{1=#1}{R}{{\ifthenelse{2=#1}{S}{T}}}}}
\newcommand{\semiring}[1]{{\ifthenelse{0=#1}{\N}{{\ifthenelse{1=#1}{S}{T}}}}}
\newcommand{\semimodule}[1]{{\ifthenelse{1=#1}{M}{N}}}
\newcommand{\bitensor}[2]{\;\!\!_{#1}\otimes_{#2}}
\newcommand{\graded}[1]{{#1}_*}
\newcommand{\reversegraded}[1]{{#1}_{-*}}
\newcommand{\coreversegraded}[1]{{#1}^{-*}}
\newcommand{\leftshiftgraded}[2]{{#1}_{*-#2}}
\newcommand{\leftshiftreversegraded}[2]{{#1}_{#2-*}}
\newcommand{\rightshiftgraded}[2]{{#1}_{*+#2}}
\newcommand{\cograded}[1]{{#1}^*}
\newcommand{\dual}{{*}}
\newcommand{\groupcompletion}[1]{#1\otimes_{\N}\Z}
\newcommand{\grading}{{*}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\corank}{\mathrm{corank}}
\newcommand{\tensor}[1]{{\ifthenelse{0=#1}{\otimes_\N\;}{{\ifthenelse{1=#1}{\otimes_{\semiring{1}}\;}{\otimes_{\semiring{1}[\Sigma_p]}}}}}}

% topology
\newcommand{\rel}[1]{\;\mathop{rel}\;#1}
\newcommand{\pathspace}{\mathbb{P}}
\newcommand{\sphere}{\mathbb{S}}
\newcommand{\site}{\mathscr{O}}
\newcommand{\homotopic}{\sim}
\newcommand{\torus}{\T}
\newcommand{\interior}{\mathop{int}}
\newcommand{\topology}[1]{\mathscr{O}_{#1}}
\newcommand{\BASIS}{\mathscr{B}}
\newcommand{\deRham}{\Omega_{\mathrm{DR}}}
\newcommand{\der}[2]{\partial_{#1}^{#2}}
\newcommand{\loopspace}{\Omega}
\newcommand{\vectorfields}[1]{\mathfrak{X}(#1)}
\newcommand{\compactification}[1]{\mathbb{S}^{#1}}
\newcommand{\horn}[1]{\Lambda^{#1}}
\newcommand{\boxhorn}[1]{\sqcup^{#1}}
\newcommand{\eilenbergmaclane}[2]{K(#1,#2)}
\newcommand{\cycles}[1]{Z_{#1}}
\newcommand{\cocycles}[1]{Z^{#1}}
\newcommand{\fibrantreplacement}{R}
\newcommand{\fibrantextension}{\eta}  
\newcommand{\nerve}{\catfont{ner}}
\newcommand{\manifold}{M}
\newcommand{\leftderived}{L}
\newcommand{\rightderived}{R}
\newcommand{\filter}[1]{{\ifthenelse{1=#1}{\mathcal{F}}{{\ifthenelse{2=#1}{\mathcal{G}}{\mathcal{H}}}}}}

% geometry
\newcommand{\transport}{\nabla}

% ditopology
\newcommand{\disphere}[2]{\mathbb{S}^{#1,#2}}
\newcommand{\dihomotopic}{\leftrightsquigarrow}
\newcommand{\direalize}[1]{\upharpoonleft\!\!{#1}\!\!\downharpoonright}
\newcommand{\realize}[1]{|{#1}|}
\newcommand{\DI}[2]{\mathbb{I}^{(#1,#2)}}
\newcommand{\DS}[2]{\mathbb{S}^{(#1,#2)}}
\newcommand{\DR}[2]{\mathbb{R}^{(#1,#2)}}
\newcommand{\quasiuniformity}[1]{\ifthenelse{1=#1}{\mathscr{U}}{\ifthenelse{2=#1}{\mathscr{V}}{\mathscr{W}}}}

% order theory
\newcommand{\graph}{\mathop{graph}}
\newcommand{\meet}{\wedge}
\newcommand{\join}{\vee}

% simplicial and cubical sets
\newcommand{\Star}{\mathrm{Star}}
\newcommand{\Link}{\mathrm{Link}}
\newcommand{\openstar}{\mathrm{star}}
\newcommand{\sing}{\catfont{sing}}
\newcommand{\cosimplicial}{\nabla}
\newcommand{\tri}{\catfont{tri}\;\!\!}
\newcommand{\qua}{\catfont{qua}\;\!\!}
\newcommand{\sd}{\catfont{sd}}
\newcommand{\ex}{\catfont{ex}}
\newcommand{\digraph}[1]{\ifthenelse{1=#1}{G}{\ifthenelse{2=#1}{H}{I}}}
\newcommand{\boxobj}[1]{[1]^{#1}}
\newcommand{\multiboxobj}[2]{[#1]^{#2}}
\newcommand{\support}{\catfont{supp}}
\newcommand{\totalization}{\catfont{tot}}
\newcommand{\decalage}{\catfont{dec}}  
\newcommand{\codiagonal}{\catfont{codiag}}  

% sheaf theory
\newcommand{\orientation}{\mathcal{O}}
\newcommand{\homsheaf}{\mathit{Hom}}
\newcommand{\constantsheaf}[1]{k_{#1}}
\newcommand{\constantcosheaf}[1]{k^{#1}}
\newcommand{\globalsections}{\Gamma}
\newcommand{\globalcosections}{\ensuremath{\reflectbox{$\Gamma$}}}
\newcommand{\sheaf}[1]{\ifthenelse{1=#1}{\mathcal{F}}{\ifthenelse{2=#1}{\mathcal{G}}{\mathcal{H}}}}
\newcommand{\connection}[1]{\ifthenelse{1=#1}{\nabla}{\ifthenelse{2=#1}{\nabla}{\nabla}}}
\newcommand{\structurecosheaf}{\mathcal{T}}
\newcommand{\cosheaf}[1]{\ifthenelse{1=#1}{\mathcal{X}}{\ifthenelse{2=#1}{\mathcal{Y}}{\mathcal{Z}}}}
\newcommand{\homologysheaf}{\mathcal{H}}

